EverAdapt: Continuous Adaptation for Dynamic Machine Fault Diagnosis Environments

Unsupervised Domain Adaptation (UDA) has emerged as a key solution in data-driven fault diagnosis, addressing domain shift where models underperform in changing environments. However, under the realm of continually changing environments, UDA tends to underperform on previously seen domains when adapting to new ones - a problem known as catastrophic forgetting. To address this limitation, we introduce the EverAdapt framework, specifically designed for continuous model adaptation in dynamic environments. Central to EverAdapt is a novel Continual Batch Normalization (CBN), which leverages source domain statistics as a reference point to standardize feature representations across domains. EverAdapt not only retains statistical information from previous domains but also adapts effectively to new scenarios. Complementing CBN, we design a class-conditional domain alignment module for effective integration of target domains, and a Sample-efficient Replay strategy to reinforce memory retention. Experiments on real-world datasets demonstrate EverAdapt superiority in maintaining robust fault diagnosis in dynamic environments. Our code is available: https://github.com/mohamedr002/EverAdapt

==> archive.tex <==
% Abstract V2: 
%% Introduce UDA for addressing domain shift in fault diagnosis.
%% Drawback of UDA in sequential adaptation under dynamic environments
%% Catastrophic forgetting problem of UDA 
%% Our framework, we first introduce class-conditional aligment to effectively adapt different domains in class-wise manner. While effective in adaptation it can still prone to forgetting problem.
%% We identify one reason for forgetting is that conventional batch norm adapt the model stastics to the current domain, making it forgets about about the previous domain. 
%% Replay has been a common solution, however, it requires a large amount of samples to become effective. 
%% Here, we introduce our CBN method to adapt all the incoming domains to a single reference stastics making it less prone to forgetting mapping and standardizing the feature represenation across domains. However, due to the difference in statistics between domains, adapting target domains to source stastics usualy cause instability issue in the performance. 
%% To address the instability, we introduce entropy regularization as minimizing entropy is a means to drive the decision boundary from learning examples, enabling the class-conditional adaptation to be more stable less noisy pseudo labels.
%% We also incorporate adaptive weighting between entropy minimization and the class-conditional adaptation, by giving a smaller weight for class-condition adaptation at the begining of the training and larger entropy weight, then we make it the opposite to favor adaptation over increasing the confidence of the classifier output. 

% Abstract V2: 
%% Introduce UDA for addressing domain shift in fault diagnosis.
%% Drawback of UDA in sequential adaptation under dynamic environments
%% Catastrophic forgetting problem of UDA 
%% Our framework, we first introduce class-conditional aligment to effectively adapt different domains in class-wise manner. While effective in adaptation it can still prone to forgetting problem.
%% We identify one reason for forgetting is that conventional batch norm adapt the model stastics to the current domain, making it forgets about about the previous domain. 
%% Replay has been a common solution, however, it requires a large amount of samples to become effective. 
%% Here, we introduce our CBN method to adapt all the incoming domains to a single reference stastics making it less prone to forgetting mapping and standardizing the feature represenation across domains. However, due to the difference in statistics between domains, adapting target domains to source stastics usualy cause instability issue in the performance. 
%% To address the instability, we introduce entropy regularization as minimizing entropy is a means to drive the decision boundary from learning examples, enabling the class-conditional adaptation to be more stable less noisy pseudo labels.
%% We also incorporate adaptive weighting between entropy minimization and the class-conditional adaptation, by giving a smaller weight for class-condition adaptation at the begining of the training



% While BatchNorm significantly improves training speed and stability, it is primarily designed for static data distributions. 
% While BN is effective suitable for static data distributions, it leads to the model quickly adapting to the current domain's statistics (\(\mu_{\text{domain}}\), \(\sigma_{\text{domain}}^2\)). Such rapid adaptation can induce catastrophic forgetting in continual learning environments, as it causes the network's normalization parameters to prioritize recent data, often neglecting information from previous domains. Consequently, there is a pronounced need for an adaptive normalization approach in environments with dynamically changing data distributions, ensuring consistent model performance across various domains.

% A key limitation of conventional Batch Normalization in continual learning contexts is its approach to domain-specific statistics. Batch Normalization normalizes network inputs based on the current domain's statistics, as illustrated by the equation:

% \begin{equation}
%     \text{BN}(x; \mu_{\text{domain}}, \sigma_{\text{domain}}^2) = \gamma \left( \frac{x - \mu_{\text{domain}}}{\sqrt{\sigma_{\text{domain}}^2 + \epsilon}} \right) + \beta
% \end{equation}

% In this context, \(\mu_{\text{domain}}\) and \(\sigma_{\text{domain}}^2\) are the mean and variance from the current domain. This can cause a loss of information about the statistical properties of previous domains in continual learning.


% While BatchNorm significantly improves training speed and stability, it is primarily designed for static data distributions. This becomes a limitation in scenarios where the data distribution is dynamic, such as in continual learning or non-stationary environments. In such settings, BatchNorm can contribute to catastrophic forgetting, a phenomenon where the network loses the information learned from previous domains. This occurs because the normalization parameters become optimized for the latest data distribution, potentially overriding patterns learned from earlier data. This challenge highlights the need for a more adaptive approach to normalization in continually evolving learning environments.


% \subsubsection{Continual Batch Norm}
% While BatchNorm significantly improves training speed and stability, it is primarily designed for static data distributions. This becomes a limitation in scenarios where the data distribution is dynamic, such as in continual learning or non-stationary environments. In such settings, BatchNorm can contribute to catastrophic forgetting, a phenomenon where the network loses the information learned from previous domains. This occurs because the normalization parameters become optimized for the latest data distribution, potentially overriding patterns learned from earlier data. This challenge highlights the need for a more adaptive approach to normalization in continually evolving learning environments.

% A straightforward strategy to combat this is to store and revisit data from past learning domains during future adaptations. However, this approach requires retaining a substantial portion of data from each previously encountered domain, which becomes impractically memory-intensive as the number of domains increases. To address this, our novel technique, Catastrophic Blocking Network (CBN), markedly enhances the efficiency of using replay samples. CBN achieves this by significantly reducing the size of replay samples needed to prevent catastrophic forgetting. We will delve into the specifics of replay samples and the workings of CBN in the following sections.

%and larger entropy weight, then we make it the opposite to favor adaptation over increasing the confidence of the classifier output. 

% Old narrative with replay being introduced as a method
% To address the catastrophic forgetting problem, we introduce a forgetting prevention module comprising two key components: Continual Batch Normalization (CBN) and Sample-efficient Replay (SR). CBN is designed to standardize the normalization process across various domains, using fixed source domain statistics. This approach helps in maintaining consistent feature representation across domains, thereby significantly reducing catastrophic forgetting. Additionally, the Sample-efficient Replay module addresses the variability in class distribution across domains. By efficiently aligning class distributions between the source and previously encountered domains, this module aids in reinforcing the model's memory and ensuring the retention of critical class-specific information.
% In industrial environments, obtaining properly labeled data is a significant challenge. Furthermore, varying working conditions in industrial equipment often lead to the domain shift problem, where a model trained on a specific dataset may demonstrate poor generalization when applied to another dataset with a different distribution. Domain Adaptation (DA) has garnered significant attention in fault diagnosis to address this issue. Prior studies \cite{lu2016deep,li2019multi,lu2021new} have focused on aligning source and target feature distributions using Maximum Mean Discrepancy (MMD) to mitigate domain shift. In a similar vein, \cite{jiao2020double,li2019deep} employ adversarial networks for distribution alignment. Improving previous works, subsequent papers introduced class-conditional alignment methods for superior adaptation performance \cite{wang2021subdomain,chen2022residual} To address the issue from another angle, \cite{wei2021weighted,zhu2020new} propose leveraging multiple source domains through a weighting scheme.
% Yet, these methods can handle for static environment with single target domain these approaches can adapt to static environments, they fail to handle dynamic environments, where models enqunter multiple domains sequantially. Moreover, by adapting to new domains they usally forget knowledge about prevoous domains 

% However, a common limitation of these existing DA methods is the assumption of complete access to the target domain during adaptation. This assumption is often unrealistic in the dynamic industrial environment, where working conditions are subject to frequent change, leading to the emergence of new target domains. Most of these methods do not incorporate a strategy for updating the model to adapt to these new target domains.

% In contrast, our approach of continual domain adaptation proposes a more realistic setting. It acknowledges the scenarios where access to the entire target domain may not be feasible and emphasizes the model's need to adapt to new target domains without catastrophic forgetting, forgetting the knowledge acquired from previously learned domains.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> narraitve_versions.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Narrative V1: Centered around CBN with all proposed details
% class-conditional, replay, CBN, entropy, adaptive weighting
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Introducing UDA's Role in Fault Diagnosis: Unsupervised Domain Adaptation (UDA) is introduced as a key method for addressing domain shifts in fault diagnosis, adapting models to various data conditions.
%% Challenges in Sequential Adaptation: However, UDA encounters drawbacks in sequential adaptation under dynamic environments, a critical aspect of fault diagnosis.
%% Catastrophic Forgetting in UDA: A major issue with UDA in these settings is catastrophic forgetting, where the model loses information about previously encountered domains while adapting to new ones.
%% Class-Conditional Alignment in Our Framework: Our framework first implements class-conditional alignment for effective domain adaptation in a class-wise manner, although it is not immune to the forgetting problem.
%% Identifying Forgetting Causes: We pinpoint that conventional batch normalization, which adapts model statistics to the current domain, contributes significantly to this forgetting, neglecting previously learned domains.
%% Limitations of Replay and Introduction of CBN: While replay is a common solution to this issue, its effectiveness hinges on a large sample size. 
%% Introduction of CBN: To enhance efficiency, we introduce the Conditional Batch Normalization (CBN) method, aligning all incoming domains to a unified reference statistic, thus reducing forgetting and standardizing feature representation across domains.
%% Addressing Performance Instability: We acknowledge that aligning different domains to a single source statistic can cause instability in performance. To counter this, we incorporate entropy regularization, which by minimizing entropy, stabilizes class-conditional adaptation and yields less noisy pseudo labels.
%% Adaptive Weighting Strategy: Further refining our approach, we integrate an adaptive weighting mechanism. This involves initially favoring entropy minimization over class-conditional adaptation, then gradually shifting this balance to enhance adaptation and boost classifier confidence as training progresses.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Narrative V2: Consider adaptation and retention goals
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%% DA's Role in Fault Diagnosis: Unsupervised Domain Adaptation (UDA) plays a key role in fault diagnosis, enabling models to adapt to diverse datasets and tackle the challenge of distribution shifts.
%% Dynamic Environment Challenge: The dynamic nature of fault diagnosis, characterized by continually emerging new target domains, requires models to efficiently adapt to these changes while retaining knowledge from past domains.
%% EverAdapt Approach Introduction: 'EverAdapt' addresses this challenge, synergizing class-conditional alignment for adaptation to new domains with class-conditional replay for knowledge retention. However, despite their effectiveness, these methods encounter hurdles due to the distribution discrepancy between domains.
%% Identifying Batch Normalization Limitations: Specifically, with such distribution shifts, we find that conventional batch normalization can be detrimental to both adaptation and retention. It tends to be domain-specific, leading to less generalizability to incoming domains and a tendency to forget about previous domains.
%% Continual Batch Norm Solution: To overcome this, we introduce the 'Continual Batch Norm', which uses source domain statistics as a reference. This innovation standardizes feature representations across domains, ensuring more effective adaptation and consistent performance across various domains.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Narrative V3: Centered around CBN, with less details about it
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Highlighting UDA's Role: UDA demonstrates significant efficacy in addressing distribution shifts essential for fault diagnosis, adapting models to varied datasets effectively.
%% Dynamic Environment Challenges: However, UDA's capabilities are tested in dynamic fault diagnosis environments, where the ever-changing nature of domain conditions poses a substantial challenge.
%% Catastrophic Forgetting Issue: A prominent issue in these dynamic settings is catastrophic forgetting, where models struggle to maintain performance across continually changing domains.
%% Introducing EverAdapt for Continual Adaptation: To address this, we introduce 'EverAdapt', a novel approach designed for continual domain adaptation in these challenging environments.
%% Central Role of Continual Batch Norm: A key component of EverAdapt is the 'Continual Batch Norm', which we introduce to address the limitations of conventional batch normalization in handling domain variability.
%% Contrasting with Conventional Batch Norm: This new batch norm method contrasts with traditional approaches by maintaining consistency across domain transitions, thus mitigating the forgetting issue.
%% Complementing with Class-Conditional Alignment: EverAdapt further complements this with class-conditional alignment, applying it both between domains and on replay samples to enhance adaptation efficiency.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Narrative V4: Centered around CBN, with less details about it
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Highlighting UDA's Role: UDA demonstrates significant efficacy in addressing distribution shifts essential for fault diagnosis, adapting models to varied datasets effectively.
%% Dynamic Environment Challenges: However, UDA's capabilities are tested in dynamic fault diagnosis environments, where the ever-changing nature of domain conditions poses a substantial challenge.
%% Catastrophic Forgetting Issue: A prominent issue in these dynamic settings is catastrophic forgetting, where models struggle to maintain performance across continually changing domains.
%% Introduce replay here as a conventional solution, we introduce our CBN as a way to reduce the memory need. 
%% Stability-plasticity problem--> More adapt more forgetting and vice versa

%% Introducing EverAdapt for Continual Adaptation: To address this, we introduce 'EverAdapt', a novel approach designed for continual domain adaptation in these challenging environments.
%% Central Role of Continual Batch Norm: A key component of EverAdapt is the 'Continual Batch Norm', which we introduce to address the limitations of conventional batch normalization in handling domain variability.
%% Contrasting with Conventional Batch Norm: This new batch norm method contrasts with traditional approaches by maintaining consistency across domain transitions, thus mitigating the forgetting issue.
%% Complementing with Class-Conditional Alignment: EverAdapt further complements this with class-conditional alignment, applying it both between domains and on replay samples to enhance adaptation efficiency.










%%% Drafts %%%

%% one idea is to introduce 
%% UDA efficacy in addressing distribution shift for fault diagnosis
%% Limitation of UDA in dynamic FD environments 
%% Catastrophic forgetting problem across domains
%% Sequential adaptation has two main challenges: (1) adapting effectively on new domains (2) forgetting knowledge of previous domains.
%% Here we introduce our everadapt approach: 
% Unlike the global alignment technique that ignore class-information, we introduce class-conditional aligment--> adaptation technique,
% Moreover, for more sample-efficient memory retention, we introduce class-conditional replay, where alignment of similar classes of the current domain and memory samples is conducted. This is far more efficient than global distribution alignment, which requires larger sample size to be effective.

%% Despite the efficacy of these, we identify one key issue that hinders both adaptation and retention.  Current conventional BN mainly focuses on adapting to the batch statistics making it overfit to the current domain. Due to the different statistics between domains, adapting each domain to its own statistics, make the model forget knowledge about previous domains, but also hinders adaptation across different domains.
%%  Introducing continual batch norm as a central component, which leverages source domain statistics as a reference point to standardize feature representations across domains.






% Abstract V2: 
%% Introduce UDA for addressing domain shift in fault diagnosis.
%% Drawback of UDA in sequential adaptation under dynamic environments
%% Catastrophic forgetting problem of UDA 
%% Our framework, we first introduce class-conditional aligment to effectively adapt different domains in class-wise manner. While effective in adaptation it can still prone to forgetting problem.
%% We identify one reason for forgetting is that conventional batch norm adapt the model stastics to the current domain, making it forgets about about the previous domain. 
%% Replay has been a common solution, however, it requires a large amount of samples to become effective. 
%% Here, we introduce our CBN method to adapt all the incoming domains to a single reference stastics making it less prone to forgetting mapping and standardizing the feature represenation across domains. However, due to the difference in statistics between domains, adapting target domains to source stastics usualy cause instability issue in the performance. 
%% To address the instability, we introduce entropy regularization as minimizing entropy is a means to drive the decision boundary from learning examples, enabling the class-conditional adaptation to be more stable less noisy pseudo labels.
%% We also incorporate adaptive weighting between entropy minimization and the class-conditional adaptation, by giving a smaller weight for class-condition adaptation at the begining of the training and larger entropy weight, then we make it the opposite to favor adaptation over increasing the confidence of the classifier output. 

% Abstract V2: 
%% Introduce UDA for addressing domain shift in fault diagnosis.
%% Drawback of UDA in sequential adaptation under dynamic environments
%% Catastrophic forgetting problem of UDA 
%% Our framework, we first introduce class-conditional aligment to effectively adapt different domains in class-wise manner. While effective in adaptation it can still prone to forgetting problem.
%% We identify one reason for forgetting is that conventional batch norm adapt the model stastics to the current domain, making it forgets about about the previous domain. 
%% Replay has been a common solution, however, it requires a large amount of samples to become effective. 
%% Here, we introduce our CBN method to adapt all the incoming domains to a single reference stastics making it less prone to forgetting mapping and standardizing the feature represenation across domains. However, due to the difference in statistics between domains, adapting target domains to source stastics usualy cause instability issue in the performance. 
%% To address the instability, we introduce entropy regularization as minimizing entropy is a means to drive the decision boundary from learning examples, enabling the class-conditional adaptation to be more stable less noisy pseudo labels.
%% We also incorporate adaptive weighting between entropy minimization and the class-conditional adaptation, by giving a smaller weight for class-condition adaptation at the begining of the training and larger entropy weight, then we make it the opposite to favor adaptation over increasing the confidence of the classifier output. 


==> utils/abstract_versions.tex <==

\section{V1} 
Unsupervised Domain Adaptation (UDA) has become a cornerstone in achieving effective data-driven fault diagnosis across industries, especially in environments characterized by changing operational conditions. However, existing UDA methodologies often struggle with sequential adaptation to multiple domains, leading to a significant issue of catastrophic forgetting. To address this limitation, we introduce the "EverAdapt" framework, specifically designed for continuous model adaptation in  dynamic environments. Central to EverAdapt is our innovative Continual Batch Normalization (CBN), which dramatically outperforms conventional Batch Normalization in mitigating the forgetting issue. Unlike traditional BN that normalizes data for each domain independently, leading to a loss of information from prior domains, CBN utilizes source domain statistics as a reference point. This approach standardizes feature representations across all domains, ensuring that the knowledge from previous domains is not just retained but also effectively utilized in new domain adaptations. This key aspect of CBN significantly reduces the problem of catastrophic forgetting, a common shortfall in sequential domain adaptation. 
Complementing CBN, EverAdapt includes a class-conditional domain alignment module for effective integration of target domains, and a Sample-efficient Replay strategy to reinforce memory retention. Together, these components make EverAdapt a powerful tool for maintaining robust fault diagnosis in dynamic operational environments, as evidenced by our empirical results that demonstrate its superiority over existing state-of-the-art methods


\section{V2} 
Unsupervised Domain Adaptation (UDA) has emerged as a key solution in data-driven fault diagnosis, addressing 'domain shift' where models underperform in dynamic environments with changing data distributions. Despite its potential, UDA often struggles in the dynamic realm of fault diagnosis, where models sequentially encounter varied domains. It tends to lose efficacy on previously seen domains while adapting to new ones—a problem known as catastrophic forgetting.
To address this limitation, we introduce the "EverAdapt" framework, specifically designed for continuous model adaptation in  dynamic environments. Central to EverAdapt is our  Continual Batch Normalization (CBN), which, unlike conventional Batch Normalization, leverages source domain statistics as a reference point to standardize feature representations across domains. This methodology not only maintains the integrity of information from previous domains but also ensures its effective application in new scenarios. Complementing CBN, EverAdapt includes a class-conditional domain alignment module for effective integration of target domains, and a Sample-efficient Replay strategy to reinforce memory retention. Together, these components make EverAdapt a powerful tool for maintaining robust fault diagnosis in dynamic operational environments.
The effectiveness of EverAdapt is validated through experiments on real-world datasets, demonstrating its superiority in maintaining robust fault diagnosis in dynamic operational environments compared to existing state-of-the-art methods


